OSEF: One-Step Evidence Fusion for Cross-Video Scene Procedure Planning

Procedure planning in instructional videos predicts actions between supplied start and goal observations (video scene procedure planning, or VSPP, in our notation). We introduce Cross-Video Scene Procedure Planning (CVSPP), which instead takes a start--goal query and candidate videos, and predicts an action sequence together with its supporting video and interval. Two challenges arise: demonstrations of the same task can support different transitions, and an early retrieval error can deprive the planner of relevant evidence. We construct a dedicated benchmark from eleven video sources, with task-specific queries, candidate sets, and linked video--interval--plan references. Its fourteen settings support a broad study of nine adapted planner families. We propose One-Step Evidence Fusion (OSEF), which retains candidate features while producing interval-conditioned planning representations. Separate boundary scores model the supporting interval, and compatible-mass decoding combines the probability of the same complete plan across overlapping intervals before selecting the output. Joint evaluation requires video, interval, and plan to match one reference example. Across four matched development-data comparisons on NIV, CrossTask, and COIN, compatible-mass decoding increases mean joint success by $2.40$--$6.79$ percentage points without retraining. On NIV, query-only controls retain plan accuracy yet sharply reduce joint success; donor-interface studies examine how VSPP models use retrieved visual states. We further identify temporal-reference sensitivity: changing only the reference projection can reverse the decoding gain, exposing an evaluation challenge for the new task.

==> evidence/coin12_full_results_047.tex <==
\FloatBarrier
\section{COIN: complete fixed-E100 results}
\label{app:coin12-full-047}
This section reports all 12 COIN~\cite{coin2019} models (four conditions, seeds 0--2) on the same 4,685 exposed VALID records. Both decisions and both reference policies reuse each model; they do not add training runs or independent samples. The task has $T=3$, $K=4$ and $M=16$ with 544 candidate intervals. Coordinates are quantized annotation proxies. Finite witnesses comprise the retained annotations, not every semantically valid answer. All conjunctions require one witness to satisfy the relevant conditions.
The fixed-E100 checkpoints were exported before reference scoring. Saved-output QA and separate scoring/recount processes completed; their metric and aggregation implementations differ but share protocol loading. Agreement verifies the stored computations, not semantic annotation completeness or physical time. The original G-score seed-0 training process exited with status 1; its recovered E100 state and subsequent successful export and scoring are retained separately, without rewriting that training failure.
Joint MAP and evidence-first use the same saved hypothesis bank. In particular, query-only success depends strongly on the decision rule; joint and evidence-first results must not be interchanged. All means and sample SDs below are recomputed from integer counts. SD describes three training seeds and is not a confidence interval.

\paragraph{Data and split.}
The official COIN training/testing split yields 14,558 TRAIN cases and 4,685 evaluation cases, with 778 action labels and horizon three. The testing-derived evaluation cohort has already been exposed during development and is reported as VALID. The corresponding eligible feature banks contain 7,551 training and 2,500 testing video IDs; these are video counts, not case counts. Candidates are constructed within each split's task pools. The same four conditions and three seeds use the same case lists.

\paragraph{Visual readout and interval coordinates.}
For each video's stored FP32 feature sequence $X\in\mathbb{R}^{L\times512}$, the readout selects rows
\begin{equation}
 r_m=\operatorname{round}_{\mathrm{NumPy}}\!\left(\frac{m(L-1)}{15}\right),
 \qquad m=0,\ldots,15.
\end{equation}
The 16 selected rows are copied without re-encoding, projection or averaging; all 16 validity entries are true. The retained source chain certifies this readout, but does not establish the original visual encoder's identity or extraction recipe. We therefore do not identify these features with the separately reconstructed NIV encoder. For an annotation window's temporal hull $[a,b]$ and video duration $d$, the proxy interval is
\begin{align}
 s&=\operatorname{clip}_{[0,15]}\!\left(\left\lfloor15a/d\right\rfloor\right),\\
 e&=\max\!\left\{s,\operatorname{clip}_{[0,15]}\!\left(\left\lceil15b/d\right\rceil\right)\right\}.
\end{align}
Intervals are inclusive: their length is $e-s+1$, and IoU at least one half requires twice the intersection length to be at least the union length. Annotation quantization and feature-row selection are separate operations; this construction does not establish feature-frame timestamp alignment.

\paragraph{Query encoding.}
The stored answer-redacted query is encoded with frozen BERT-base~\cite{bert2019}: 768 hidden dimensions, 12 layers, 12 attention heads and a 30,522-token vocabulary. Tokenization adds CLS/SEP, uses no truncation, and retains 2--512 valid tokens. Eager attention uses FP32 without AMP or TF32. The saved FP32 last-hidden token vectors are summed sequentially in FP64, divided by the valid-token count, and cast to FP32. This 768-dimensional query mean includes CLS/SEP and excludes padding; it is neither a pooler output nor the CLS vector alone. Training reads this fixed cache.

\paragraph{Training budget and hypothesis evaluation.}
Each of the 12 retained E100 states records 182,000 optimizer updates and 1,455,800 case exposures across 100 epochs. A batch of eight gives 1,820 steps per epoch, including the final six cases. AdamW~\cite{loshchilov2019adamw} uses learning rate $10^{-4}$, $(\beta_1,\beta_2)=(0.9,0.999)$, $\epsilon=10^{-8}$ and weight decay $0.01$, with FP32 gradient-norm clipping at one. Microbatch size is eight and planner chunk size is 16, with nonreentrant activation checkpointing and the MATH attention backend. Epoch ordering uses a fixed shuffle seeded by the epoch index. Final E100 checkpoints are used without validation-based epoch selection.

Evidence probabilities normalize over all $H=4\times16\times17/2=544$ candidate intervals during training. For the planning term, training evaluates every interval on the canonical witness video whose proxy IoU is at least one half, and computes the accepted-event mass by log-sum-exp across this complete accepted subset. The subset is not sampled; padding entries are masked out. Training therefore does not forward the planner on all 544 conditions for every case. Public inference does enumerate all 544 planner conditions, from which joint MAP and evidence-first decisions share the same hypothesis bank. These are matched budgets within COIN; the different data volume, action vocabulary and visual inputs preclude claiming equal training computation across COIN and NIV.

\begin{table*}[!t]\centering\footnotesize\setlength{\tabcolsep}{3pt}
\begin{tabular}{lllrrrrr}\toprule
Decision & Reference & Condition & $V$ & $P$ & $VP$ & $VI_{.5}$ & $J_{.5}$ \\\midrule
joint & canonical & G-score & $34.54\pm0.28$ & $63.29\pm0.03$ & $22.70\pm0.04$ & $16.62\pm0.13$ & $11.49\pm0.23$ \\
joint & canonical & G-uniform & $34.53\pm0.42$ & $62.58\pm0.76$ & $22.40\pm0.47$ & $16.46\pm0.26$ & $11.38\pm0.27$ \\
joint & canonical & W-score & $35.01\pm0.43$ & $62.61\pm0.42$ & $22.65\pm0.48$ & $16.84\pm0.29$ & $11.68\pm0.17$ \\
joint & canonical & query-only & $25.15\pm0.26$ & $65.23\pm0.61$ & $15.94\pm0.20$ & $11.65\pm0.31$ & $8.04\pm0.30$ \\
\addlinespace[2pt]
joint & finite & G-score & $60.15\pm0.50$ & $70.00\pm0.27$ & $42.93\pm0.28$ & $33.74\pm0.58$ & $25.12\pm0.73$ \\
joint & finite & G-uniform & $59.59\pm0.47$ & $69.26\pm0.93$ & $42.44\pm0.56$ & $33.28\pm0.70$ & $24.92\pm0.29$ \\
joint & finite & W-score & $60.31\pm0.26$ & $69.07\pm0.59$ & $42.71\pm1.14$ & $33.80\pm0.34$ & $24.99\pm0.55$ \\
joint & finite & query-only & $44.20\pm0.08$ & $72.29\pm0.70$ & $31.50\pm0.21$ & $23.88\pm0.60$ & $17.99\pm0.69$ \\
\addlinespace[2pt]
E-first & canonical & G-score & $34.58\pm0.32$ & $62.85\pm0.25$ & $22.45\pm0.11$ & $16.71\pm0.31$ & $11.41\pm0.43$ \\
E-first & canonical & G-uniform & $34.51\pm0.30$ & $62.04\pm0.40$ & $22.28\pm0.22$ & $16.54\pm0.24$ & $11.37\pm0.23$ \\
E-first & canonical & W-score & $35.19\pm0.33$ & $61.70\pm0.67$ & $22.46\pm0.41$ & $16.75\pm0.15$ & $11.49\pm0.05$ \\
E-first & canonical & query-only & $25.02\pm0.00$ & $56.62\pm1.94$ & $13.68\pm0.45$ & $0.02\pm0.00$ & $0.02\pm0.00$ \\
\addlinespace[2pt]
E-first & finite & G-score & $60.23\pm0.67$ & $69.55\pm0.26$ & $42.69\pm0.24$ & $33.94\pm0.83$ & $24.97\pm0.88$ \\
E-first & finite & G-uniform & $59.59\pm0.45$ & $68.80\pm0.64$ & $42.14\pm0.26$ & $33.39\pm0.76$ & $24.80\pm0.44$ \\
E-first & finite & W-score & $60.44\pm0.59$ & $68.17\pm0.84$ & $42.30\pm1.34$ & $33.63\pm0.40$ & $24.67\pm0.63$ \\
E-first & finite & query-only & $43.95\pm0.00$ & $63.26\pm2.03$ & $27.37\pm1.08$ & $0.15\pm0.00$ & $0.15\pm0.00$ \\
\addlinespace[2pt]
\bottomrule\end{tabular}
\caption{All COIN conditions: percentage mean $\pm$ sample SD across seeds 0--2, denominator 4,685 for every seed. Canonical and finite policies rescore the same predictions.}
\label{tab:coin12-all-summary-047}\end{table*}
\begin{table*}[!t]\centering\footnotesize\setlength{\tabcolsep}{5pt}
\begin{tabular}{llrrrrrr}\toprule
Reference & Condition & Seed & $V$ & $P$ & $VP$ & $VI_{.5}$ & $J_{.5}$ \\\midrule
canonical & G-score & 0 & 1605 & 2967 & 1065 & 781 & 551 \\
canonical & G-score & 1 & 1631 & 2965 & 1064 & 783 & 532 \\
canonical & G-score & 2 & 1619 & 2964 & 1061 & 772 & 532 \\
\addlinespace[1pt]
canonical & G-uniform & 0 & 1595 & 2953 & 1056 & 757 & 546 \\
canonical & G-uniform & 1 & 1626 & 2891 & 1025 & 778 & 521 \\
canonical & G-uniform & 2 & 1632 & 2952 & 1068 & 778 & 532 \\
\addlinespace[1pt]
canonical & W-score & 0 & 1623 & 2937 & 1056 & 792 & 538 \\
canonical & W-score & 1 & 1635 & 2912 & 1042 & 801 & 554 \\
canonical & W-score & 2 & 1662 & 2951 & 1086 & 774 & 549 \\
\addlinespace[1pt]
canonical & query-only & 0 & 1165 & 3027 & 736 & 549 & 378 \\
canonical & query-only & 1 & 1189 & 3084 & 752 & 558 & 390 \\
canonical & query-only & 2 & 1181 & 3057 & 753 & 530 & 362 \\
\addlinespace[1pt]
finite & G-score & 0 & 2842 & 3266 & 2026 & 1612 & 1216 \\
finite & G-score & 1 & 2817 & 3281 & 2007 & 1566 & 1158 \\
finite & G-score & 2 & 2795 & 3291 & 2001 & 1564 & 1156 \\
\addlinespace[1pt]
finite & G-uniform & 0 & 2768 & 3276 & 2005 & 1524 & 1157 \\
finite & G-uniform & 1 & 2811 & 3195 & 1958 & 1589 & 1183 \\
finite & G-uniform & 2 & 2796 & 3264 & 2002 & 1565 & 1162 \\
\addlinespace[1pt]
finite & W-score & 0 & 2838 & 3241 & 2040 & 1599 & 1185 \\
finite & W-score & 1 & 2814 & 3206 & 1940 & 1567 & 1141 \\
finite & W-score & 2 & 2825 & 3261 & 2023 & 1584 & 1187 \\
\addlinespace[1pt]
finite & query-only & 0 & 2069 & 3356 & 1474 & 1145 & 867 \\
finite & query-only & 1 & 2068 & 3421 & 1486 & 1122 & 855 \\
finite & query-only & 2 & 2075 & 3384 & 1467 & 1089 & 806 \\
\addlinespace[1pt]
\bottomrule\end{tabular}
\caption{COIN joint MAP: exact per-seed success counts, each out of 4,685. No seed, condition or reference policy is omitted.}
\label{tab:coin12-counts-joint-047}\end{table*}
\begin{table*}[!t]\centering\footnotesize\setlength{\tabcolsep}{5pt}
\begin{tabular}{llrrrrrr}\toprule
Reference & Condition & Seed & $V$ & $P$ & $VP$ & $VI_{.5}$ & $J_{.5}$ \\\midrule
canonical & G-score & 0 & 1618 & 2954 & 1057 & 799 & 557 \\
canonical & G-score & 1 & 1636 & 2931 & 1047 & 779 & 519 \\
canonical & G-score & 2 & 1606 & 2948 & 1051 & 771 & 527 \\
\addlinespace[1pt]
canonical & G-uniform & 0 & 1603 & 2911 & 1048 & 770 & 545 \\
canonical & G-uniform & 1 & 1631 & 2886 & 1032 & 788 & 524 \\
canonical & G-uniform & 2 & 1617 & 2923 & 1051 & 767 & 529 \\
\addlinespace[1pt]
canonical & W-score & 0 & 1643 & 2919 & 1063 & 784 & 536 \\
canonical & W-score & 1 & 1637 & 2857 & 1030 & 792 & 541 \\
canonical & W-score & 2 & 1666 & 2896 & 1064 & 778 & 538 \\
\addlinespace[1pt]
canonical & query-only & 0 & 1172 & 2552 & 618 & 1 & 1 \\
canonical & query-only & 1 & 1172 & 2677 & 646 & 1 & 1 \\
canonical & query-only & 2 & 1172 & 2729 & 659 & 1 & 1 \\
\addlinespace[1pt]
finite & G-score & 0 & 2848 & 3254 & 2013 & 1635 & 1217 \\
finite & G-score & 1 & 2830 & 3249 & 1993 & 1569 & 1144 \\
finite & G-score & 2 & 2787 & 3272 & 1994 & 1566 & 1148 \\
\addlinespace[1pt]
finite & G-uniform & 0 & 2777 & 3239 & 1985 & 1533 & 1145 \\
finite & G-uniform & 1 & 2816 & 3189 & 1961 & 1603 & 1185 \\
finite & G-uniform & 2 & 2782 & 3242 & 1977 & 1557 & 1156 \\
\addlinespace[1pt]
finite & W-score & 0 & 2858 & 3224 & 2041 & 1585 & 1180 \\
finite & W-score & 1 & 2803 & 3149 & 1916 & 1554 & 1123 \\
finite & W-score & 2 & 2834 & 3208 & 1988 & 1588 & 1164 \\
\addlinespace[1pt]
finite & query-only & 0 & 2059 & 2858 & 1224 & 7 & 7 \\
finite & query-only & 1 & 2059 & 2990 & 1307 & 7 & 7 \\
finite & query-only & 2 & 2059 & 3043 & 1316 & 7 & 7 \\
\addlinespace[1pt]
\bottomrule\end{tabular}
\caption{COIN evidence-first: exact per-seed success counts, each out of 4,685. No seed, condition or reference policy is omitted.}
\label{tab:coin12-counts-Efirst-047}\end{table*}
\begin{table*}[!t]\centering\footnotesize\setlength{\tabcolsep}{5pt}
\begin{tabular}{lllrrrr}\toprule
Reference & G-score minus & Axis & $\Delta n_0$ & $\Delta n_1$ & $\Delta n_2$ & Mean $\pm$ SD (pp) \\\midrule
canonical & G-uniform & V & 10 & 5 & -13 & $+0.01\pm0.26$ \\
canonical & G-uniform & P & 14 & 74 & 12 & $+0.71\pm0.75$ \\
canonical & G-uniform & VP & 9 & 39 & -7 & $+0.29\pm0.50$ \\
canonical & G-uniform & $VI_{.5}$ & 24 & 5 & -6 & $+0.16\pm0.32$ \\
canonical & G-uniform & $J_{.5}$ & 5 & 11 & 0 & $+0.11\pm0.12$ \\
\addlinespace[2pt]
canonical & W-score & V & -18 & -4 & -43 & $-0.46\pm0.42$ \\
canonical & W-score & P & 30 & 53 & 13 & $+0.68\pm0.43$ \\
canonical & W-score & VP & 9 & 22 & -25 & $+0.04\pm0.52$ \\
canonical & W-score & $VI_{.5}$ & -11 & -18 & -2 & $-0.22\pm0.17$ \\
canonical & W-score & $J_{.5}$ & 13 & -22 & -17 & $-0.18\pm0.40$ \\
\addlinespace[2pt]
canonical & query-only & V & 440 & 442 & 438 & $+9.39\pm0.04$ \\
canonical & query-only & P & -60 & -119 & -93 & $-1.94\pm0.63$ \\
canonical & query-only & VP & 329 & 312 & 308 & $+6.75\pm0.24$ \\
canonical & query-only & $VI_{.5}$ & 232 & 225 & 242 & $+4.97\pm0.18$ \\
canonical & query-only & $J_{.5}$ & 173 & 142 & 170 & $+3.45\pm0.36$ \\
\addlinespace[2pt]
finite & G-uniform & V & 74 & 6 & -1 & $+0.56\pm0.88$ \\
finite & G-uniform & P & -10 & 86 & 27 & $+0.73\pm1.03$ \\
finite & G-uniform & VP & 21 & 49 & -1 & $+0.49\pm0.53$ \\
finite & G-uniform & $VI_{.5}$ & 88 & -23 & -1 & $+0.46\pm1.25$ \\
finite & G-uniform & $J_{.5}$ & 59 & -25 & -6 & $+0.20\pm0.94$ \\
\addlinespace[2pt]
finite & W-score & V & 4 & 3 & -30 & $-0.16\pm0.41$ \\
finite & W-score & P & 25 & 75 & 30 & $+0.92\pm0.59$ \\
finite & W-score & VP & -14 & 67 & -22 & $+0.22\pm1.05$ \\
finite & W-score & $VI_{.5}$ & 13 & -1 & -20 & $-0.06\pm0.35$ \\
finite & W-score & $J_{.5}$ & 31 & 17 & -31 & $+0.12\pm0.69$ \\
\addlinespace[2pt]
finite & query-only & V & 773 & 749 & 720 & $+15.95\pm0.57$ \\
finite & query-only & P & -90 & -140 & -93 & $-2.30\pm0.60$ \\
finite & query-only & VP & 552 & 521 & 534 & $+11.43\pm0.33$ \\
finite & query-only & $VI_{.5}$ & 467 & 444 & 475 & $+9.86\pm0.34$ \\
finite & query-only & $J_{.5}$ & 349 & 303 & 350 & $+7.13\pm0.57$ \\
\addlinespace[2pt]
\bottomrule\end{tabular}
\caption{COIN joint MAP: all paired metric differences, G-score minus each control, across the same 4,685 records per seed. Negative and zero differences are retained.}
\label{tab:coin12-deltas-joint-047}\end{table*}
\begin{table*}[!t]\centering\footnotesize\setlength{\tabcolsep}{5pt}
\begin{tabular}{llrrrrrr}\toprule
Control & Axis & Seed & Both & Score only & Control only & Neither & $\Delta n$ \\\midrule
G-uniform & V & 0 & 1137 & 468 & 458 & 2622 & 10 \\
G-uniform & V & 1 & 1176 & 455 & 450 & 2604 & 5 \\
G-uniform & V & 2 & 1152 & 467 & 480 & 2586 & -13 \\
G-uniform & P & 0 & 2531 & 436 & 422 & 1296 & 14 \\
G-uniform & P & 1 & 2480 & 485 & 411 & 1309 & 74 \\
G-uniform & P & 2 & 2542 & 422 & 410 & 1311 & 12 \\
G-uniform & VP & 0 & 669 & 396 & 387 & 3233 & 9 \\
G-uniform & VP & 1 & 658 & 406 & 367 & 3254 & 39 \\
G-uniform & VP & 2 & 662 & 399 & 406 & 3218 & -7 \\
G-uniform & $VI_{.5}$ & 0 & 479 & 302 & 278 & 3626 & 24 \\
G-uniform & $VI_{.5}$ & 1 & 485 & 298 & 293 & 3609 & 5 \\
G-uniform & $VI_{.5}$ & 2 & 485 & 287 & 293 & 3620 & -6 \\
G-uniform & $J_{.5}$ & 0 & 324 & 227 & 222 & 3912 & 5 \\
G-uniform & $J_{.5}$ & 1 & 294 & 238 & 227 & 3926 & 11 \\
G-uniform & $J_{.5}$ & 2 & 311 & 221 & 221 & 3932 & 0 \\
\addlinespace[2pt]
W-score & V & 0 & 1125 & 480 & 498 & 2582 & -18 \\
W-score & V & 1 & 1133 & 498 & 502 & 2552 & -4 \\
W-score & V & 2 & 1126 & 493 & 536 & 2530 & -43 \\
W-score & P & 0 & 2504 & 463 & 433 & 1285 & 30 \\
W-score & P & 1 & 2489 & 476 & 423 & 1297 & 53 \\
W-score & P & 2 & 2522 & 442 & 429 & 1292 & 13 \\
W-score & VP & 0 & 652 & 413 & 404 & 3216 & 9 \\
W-score & VP & 1 & 644 & 420 & 398 & 3223 & 22 \\
W-score & VP & 2 & 643 & 418 & 443 & 3181 & -25 \\
W-score & $VI_{.5}$ & 0 & 474 & 307 & 318 & 3586 & -11 \\
W-score & $VI_{.5}$ & 1 & 468 & 315 & 333 & 3569 & -18 \\
W-score & $VI_{.5}$ & 2 & 453 & 319 & 321 & 3592 & -2 \\
W-score & $J_{.5}$ & 0 & 299 & 252 & 239 & 3895 & 13 \\
W-score & $J_{.5}$ & 1 & 290 & 242 & 264 & 3889 & -22 \\
W-score & $J_{.5}$ & 2 & 297 & 235 & 252 & 3901 & -17 \\
\addlinespace[2pt]
query-only & V & 0 & 401 & 1204 & 764 & 2316 & 440 \\
query-only & V & 1 & 423 & 1208 & 766 & 2288 & 442 \\
query-only & V & 2 & 433 & 1186 & 748 & 2318 & 438 \\
query-only & P & 0 & 2568 & 399 & 459 & 1259 & -60 \\
query-only & P & 1 & 2634 & 331 & 450 & 1270 & -119 \\
query-only & P & 2 & 2614 & 350 & 443 & 1278 & -93 \\
query-only & VP & 0 & 231 & 834 & 505 & 3115 & 329 \\
query-only & VP & 1 & 231 & 833 & 521 & 3100 & 312 \\
query-only & VP & 2 & 247 & 814 & 506 & 3118 & 308 \\
query-only & $VI_{.5}$ & 0 & 120 & 661 & 429 & 3475 & 232 \\
query-only & $VI_{.5}$ & 1 & 123 & 660 & 435 & 3467 & 225 \\
query-only & $VI_{.5}$ & 2 & 118 & 654 & 412 & 3501 & 242 \\
query-only & $J_{.5}$ & 0 & 85 & 466 & 293 & 3841 & 173 \\
query-only & $J_{.5}$ & 1 & 78 & 454 & 312 & 3841 & 142 \\
query-only & $J_{.5}$ & 2 & 75 & 457 & 287 & 3866 & 170 \\
\addlinespace[2pt]
\bottomrule\end{tabular}
\caption{COIN joint MAP, canonical reference: all paired four-cell counts for G-score versus each control. Each row sums to 4,685; $\Delta n$ is score-only minus control-only. No case independence or confirmatory significance is inferred.}
\label{tab:coin12-fourcell-joint-canonical-047}\end{table*}
\begin{table*}[!t]\centering\footnotesize\setlength{\tabcolsep}{5pt}
\begin{tabular}{llrrrrrr}\toprule
Control & Axis & Seed & Both & Score only & Control only & Neither & $\Delta n$ \\\midrule
G-uniform & V & 0 & 2444 & 398 & 324 & 1519 & 74 \\
G-uniform & V & 1 & 2438 & 379 & 373 & 1495 & 6 \\
G-uniform & V & 2 & 2402 & 393 & 394 & 1496 & -1 \\
G-uniform & P & 0 & 2887 & 379 & 389 & 1030 & -10 \\
G-uniform & P & 1 & 2834 & 447 & 361 & 1043 & 86 \\
G-uniform & P & 2 & 2907 & 384 & 357 & 1037 & 27 \\
G-uniform & VP & 0 & 1615 & 411 & 390 & 2269 & 21 \\
G-uniform & VP & 1 & 1545 & 462 & 413 & 2265 & 49 \\
G-uniform & VP & 2 & 1584 & 417 & 418 & 2266 & -1 \\
G-uniform & $VI_{.5}$ & 0 & 1134 & 478 & 390 & 2683 & 88 \\
G-uniform & $VI_{.5}$ & 1 & 1115 & 451 & 474 & 2645 & -23 \\
G-uniform & $VI_{.5}$ & 2 & 1112 & 452 & 453 & 2668 & -1 \\
G-uniform & $J_{.5}$ & 0 & 812 & 404 & 345 & 3124 & 59 \\
G-uniform & $J_{.5}$ & 1 & 753 & 405 & 430 & 3097 & -25 \\
G-uniform & $J_{.5}$ & 2 & 797 & 359 & 365 & 3164 & -6 \\
\addlinespace[2pt]
W-score & V & 0 & 2453 & 389 & 385 & 1458 & 4 \\
W-score & V & 1 & 2410 & 407 & 404 & 1464 & 3 \\
W-score & V & 2 & 2403 & 392 & 422 & 1468 & -30 \\
W-score & P & 0 & 2852 & 414 & 389 & 1030 & 25 \\
W-score & P & 1 & 2826 & 455 & 380 & 1024 & 75 \\
W-score & P & 2 & 2887 & 404 & 374 & 1020 & 30 \\
W-score & VP & 0 & 1606 & 420 & 434 & 2225 & -14 \\
W-score & VP & 1 & 1541 & 466 & 399 & 2279 & 67 \\
W-score & VP & 2 & 1564 & 437 & 459 & 2225 & -22 \\
W-score & $VI_{.5}$ & 0 & 1148 & 464 & 451 & 2622 & 13 \\
W-score & $VI_{.5}$ & 1 & 1065 & 501 & 502 & 2617 & -1 \\
W-score & $VI_{.5}$ & 2 & 1096 & 468 & 488 & 2633 & -20 \\
W-score & $J_{.5}$ & 0 & 815 & 401 & 370 & 3099 & 31 \\
W-score & $J_{.5}$ & 1 & 727 & 431 & 414 & 3113 & 17 \\
W-score & $J_{.5}$ & 2 & 772 & 384 & 415 & 3114 & -31 \\
\addlinespace[2pt]
query-only & V & 0 & 1476 & 1366 & 593 & 1250 & 773 \\
query-only & V & 1 & 1464 & 1353 & 604 & 1264 & 749 \\
query-only & V & 2 & 1472 & 1323 & 603 & 1287 & 720 \\
query-only & P & 0 & 2935 & 331 & 421 & 998 & -90 \\
query-only & P & 1 & 3014 & 267 & 407 & 997 & -140 \\
query-only & P & 2 & 2994 & 297 & 390 & 1004 & -93 \\
query-only & VP & 0 & 981 & 1045 & 493 & 2166 & 552 \\
query-only & VP & 1 & 991 & 1016 & 495 & 2183 & 521 \\
query-only & VP & 2 & 981 & 1020 & 486 & 2198 & 534 \\
query-only & $VI_{.5}$ & 0 & 498 & 1114 & 647 & 2426 & 467 \\
query-only & $VI_{.5}$ & 1 & 475 & 1091 & 647 & 2472 & 444 \\
query-only & $VI_{.5}$ & 2 & 464 & 1100 & 625 & 2496 & 475 \\
query-only & $J_{.5}$ & 0 & 378 & 838 & 489 & 2980 & 349 \\
query-only & $J_{.5}$ & 1 & 348 & 810 & 507 & 3020 & 303 \\
query-only & $J_{.5}$ & 2 & 332 & 824 & 474 & 3055 & 350 \\
\addlinespace[2pt]
\bottomrule\end{tabular}
\caption{COIN joint MAP, finite reference: all paired four-cell counts for G-score versus each control. Each row sums to 4,685; $\Delta n$ is score-only minus control-only. No case independence or confirmatory significance is inferred.}
\label{tab:coin12-fourcell-joint-finite-047}\end{table*}
\begin{table*}[!t]\centering\footnotesize\setlength{\tabcolsep}{5pt}
\begin{tabular}{lllrrrr}\toprule
Reference & G-score minus & Axis & $\Delta n_0$ & $\Delta n_1$ & $\Delta n_2$ & Mean $\pm$ SD (pp) \\\midrule
canonical & G-uniform & V & 15 & 5 & -11 & $+0.06\pm0.28$ \\
canonical & G-uniform & P & 43 & 45 & 25 & $+0.80\pm0.24$ \\
canonical & G-uniform & VP & 9 & 15 & 0 & $+0.17\pm0.16$ \\
canonical & G-uniform & $VI_{.5}$ & 29 & -9 & 4 & $+0.17\pm0.41$ \\
canonical & G-uniform & $J_{.5}$ & 12 & -5 & -2 & $+0.04\pm0.19$ \\
\addlinespace[2pt]
canonical & W-score & V & -25 & -1 & -60 & $-0.61\pm0.63$ \\
canonical & W-score & P & 35 & 74 & 52 & $+1.15\pm0.42$ \\
canonical & W-score & VP & -6 & 17 & -13 & $-0.01\pm0.34$ \\
canonical & W-score & $VI_{.5}$ & 15 & -13 & -7 & $-0.04\pm0.31$ \\
canonical & W-score & $J_{.5}$ & 21 & -22 & -11 & $-0.09\pm0.48$ \\
\addlinespace[2pt]
canonical & query-only & V & 446 & 464 & 434 & $+9.56\pm0.32$ \\
canonical & query-only & P & 402 & 254 & 219 & $+6.23\pm2.07$ \\
canonical & query-only & VP & 439 & 401 & 392 & $+8.77\pm0.53$ \\
canonical & query-only & $VI_{.5}$ & 798 & 778 & 770 & $+16.69\pm0.31$ \\
canonical & query-only & $J_{.5}$ & 556 & 518 & 526 & $+11.38\pm0.43$ \\
\addlinespace[2pt]
finite & G-uniform & V & 71 & 14 & 5 & $+0.64\pm0.76$ \\
finite & G-uniform & P & 15 & 60 & 30 & $+0.75\pm0.49$ \\
finite & G-uniform & VP & 28 & 32 & 17 & $+0.55\pm0.17$ \\
finite & G-uniform & $VI_{.5}$ & 102 & -34 & 9 & $+0.55\pm1.48$ \\
finite & G-uniform & $J_{.5}$ & 72 & -41 & -8 & $+0.16\pm1.24$ \\
\addlinespace[2pt]
finite & W-score & V & -10 & 27 & -47 & $-0.21\pm0.79$ \\
finite & W-score & P & 30 & 100 & 64 & $+1.38\pm0.75$ \\
finite & W-score & VP & -28 & 77 & 6 & $+0.39\pm1.14$ \\
finite & W-score & $VI_{.5}$ & 50 & 15 & -22 & $+0.31\pm0.77$ \\
finite & W-score & $J_{.5}$ & 37 & 21 & -16 & $+0.30\pm0.58$ \\
\addlinespace[2pt]
finite & query-only & V & 789 & 771 & 728 & $+16.28\pm0.67$ \\
finite & query-only & P & 396 & 259 & 229 & $+6.29\pm1.90$ \\
finite & query-only & VP & 789 & 686 & 678 & $+15.32\pm1.32$ \\
finite & query-only & $VI_{.5}$ & 1628 & 1562 & 1559 & $+33.79\pm0.83$ \\
finite & query-only & $J_{.5}$ & 1210 & 1137 & 1141 & $+24.82\pm0.88$ \\
\addlinespace[2pt]
\bottomrule\end{tabular}
\caption{COIN evidence-first: all paired metric differences, G-score minus each control, across the same 4,685 records per seed. Negative and zero differences are retained.}
\label{tab:coin12-deltas-Efirst-047}\end{table*}
\begin{table*}[!t]\centering\footnotesize\setlength{\tabcolsep}{5pt}
\begin{tabular}{llrrrrrr}\toprule
Control & Axis & Seed & Both & Score only & Control only & Neither & $\Delta n$ \\\midrule
G-uniform & V & 0 & 1163 & 455 & 440 & 2627 & 15 \\
G-uniform & V & 1 & 1205 & 431 & 426 & 2623 & 5 \\
G-uniform & V & 2 & 1156 & 450 & 461 & 2618 & -11 \\
G-uniform & P & 0 & 2488 & 466 & 423 & 1308 & 43 \\
G-uniform & P & 1 & 2447 & 484 & 439 & 1315 & 45 \\
G-uniform & P & 2 & 2516 & 432 & 407 & 1330 & 25 \\
G-uniform & VP & 0 & 664 & 393 & 384 & 3244 & 9 \\
G-uniform & VP & 1 & 661 & 386 & 371 & 3267 & 15 \\
G-uniform & VP & 2 & 660 & 391 & 391 & 3243 & 0 \\
G-uniform & $VI_{.5}$ & 0 & 500 & 299 & 270 & 3616 & 29 \\
G-uniform & $VI_{.5}$ & 1 & 491 & 288 & 297 & 3609 & -9 \\
G-uniform & $VI_{.5}$ & 2 & 487 & 284 & 280 & 3634 & 4 \\
G-uniform & $J_{.5}$ & 0 & 322 & 235 & 223 & 3905 & 12 \\
G-uniform & $J_{.5}$ & 1 & 292 & 227 & 232 & 3934 & -5 \\
G-uniform & $J_{.5}$ & 2 & 308 & 219 & 221 & 3937 & -2 \\
\addlinespace[2pt]
W-score & V & 0 & 1137 & 481 & 506 & 2561 & -25 \\
W-score & V & 1 & 1145 & 491 & 492 & 2557 & -1 \\
W-score & V & 2 & 1136 & 470 & 530 & 2549 & -60 \\
W-score & P & 0 & 2472 & 482 & 447 & 1284 & 35 \\
W-score & P & 1 & 2427 & 504 & 430 & 1324 & 74 \\
W-score & P & 2 & 2462 & 486 & 434 & 1303 & 52 \\
W-score & VP & 0 & 649 & 408 & 414 & 3214 & -6 \\
W-score & VP & 1 & 637 & 410 & 393 & 3245 & 17 \\
W-score & VP & 2 & 627 & 424 & 437 & 3197 & -13 \\
W-score & $VI_{.5}$ & 0 & 476 & 323 & 308 & 3578 & 15 \\
W-score & $VI_{.5}$ & 1 & 473 & 306 & 319 & 3587 & -13 \\
W-score & $VI_{.5}$ & 2 & 458 & 313 & 320 & 3594 & -7 \\
W-score & $J_{.5}$ & 0 & 296 & 261 & 240 & 3888 & 21 \\
W-score & $J_{.5}$ & 1 & 287 & 232 & 254 & 3912 & -22 \\
W-score & $J_{.5}$ & 2 & 295 & 232 & 243 & 3915 & -11 \\
\addlinespace[2pt]
query-only & V & 0 & 408 & 1210 & 764 & 2303 & 446 \\
query-only & V & 1 & 421 & 1215 & 751 & 2298 & 464 \\
query-only & V & 2 & 433 & 1173 & 739 & 2340 & 434 \\
query-only & P & 0 & 2116 & 838 & 436 & 1295 & 402 \\
query-only & P & 1 & 2273 & 658 & 404 & 1350 & 254 \\
query-only & P & 2 & 2298 & 650 & 431 & 1306 & 219 \\
query-only & VP & 0 & 196 & 861 & 422 & 3206 & 439 \\
query-only & VP & 1 & 201 & 846 & 445 & 3193 & 401 \\
query-only & VP & 2 & 210 & 841 & 449 & 3185 & 392 \\
query-only & $VI_{.5}$ & 0 & 0 & 799 & 1 & 3885 & 798 \\
query-only & $VI_{.5}$ & 1 & 0 & 779 & 1 & 3905 & 778 \\
query-only & $VI_{.5}$ & 2 & 0 & 771 & 1 & 3913 & 770 \\
query-only & $J_{.5}$ & 0 & 0 & 557 & 1 & 4127 & 556 \\
query-only & $J_{.5}$ & 1 & 0 & 519 & 1 & 4165 & 518 \\
query-only & $J_{.5}$ & 2 & 0 & 527 & 1 & 4157 & 526 \\
\addlinespace[2pt]
\bottomrule\end{tabular}
\caption{COIN evidence-first, canonical reference: all paired four-cell counts for G-score versus each control. Each row sums to 4,685; $\Delta n$ is score-only minus control-only. No case independence or confirmatory significance is inferred.}
\label{tab:coin12-fourcell-Efirst-canonical-047}\end{table*}
\begin{table*}[!t]\centering\footnotesize\setlength{\tabcolsep}{5pt}
\begin{tabular}{llrrrrrr}\toprule
Control & Axis & Seed & Both & Score only & Control only & Neither & $\Delta n$ \\\midrule
G-uniform & V & 0 & 2472 & 376 & 305 & 1532 & 71 \\
G-uniform & V & 1 & 2462 & 368 & 354 & 1501 & 14 \\
G-uniform & V & 2 & 2409 & 378 & 373 & 1525 & 5 \\
G-uniform & P & 0 & 2845 & 409 & 394 & 1037 & 15 \\
G-uniform & P & 1 & 2799 & 450 & 390 & 1046 & 60 \\
G-uniform & P & 2 & 2881 & 391 & 361 & 1052 & 30 \\
G-uniform & VP & 0 & 1596 & 417 & 389 & 2283 & 28 \\
G-uniform & VP & 1 & 1546 & 447 & 415 & 2277 & 32 \\
G-uniform & VP & 2 & 1581 & 413 & 396 & 2295 & 17 \\
G-uniform & $VI_{.5}$ & 0 & 1164 & 471 & 369 & 2681 & 102 \\
G-uniform & $VI_{.5}$ & 1 & 1130 & 439 & 473 & 2643 & -34 \\
G-uniform & $VI_{.5}$ & 2 & 1122 & 444 & 435 & 2684 & 9 \\
G-uniform & $J_{.5}$ & 0 & 801 & 416 & 344 & 3124 & 72 \\
G-uniform & $J_{.5}$ & 1 & 750 & 394 & 435 & 3106 & -41 \\
G-uniform & $J_{.5}$ & 2 & 798 & 350 & 358 & 3179 & -8 \\
\addlinespace[2pt]
W-score & V & 0 & 2466 & 382 & 392 & 1445 & -10 \\
W-score & V & 1 & 2425 & 405 & 378 & 1477 & 27 \\
W-score & V & 2 & 2411 & 376 & 423 & 1475 & -47 \\
W-score & P & 0 & 2816 & 438 & 408 & 1023 & 30 \\
W-score & P & 1 & 2764 & 485 & 385 & 1051 & 100 \\
W-score & P & 2 & 2829 & 443 & 379 & 1034 & 64 \\
W-score & VP & 0 & 1595 & 418 & 446 & 2226 & -28 \\
W-score & VP & 1 & 1521 & 472 & 395 & 2297 & 77 \\
W-score & VP & 2 & 1535 & 459 & 453 & 2238 & 6 \\
W-score & $VI_{.5}$ & 0 & 1157 & 478 & 428 & 2622 & 50 \\
W-score & $VI_{.5}$ & 1 & 1071 & 498 & 483 & 2633 & 15 \\
W-score & $VI_{.5}$ & 2 & 1098 & 468 & 490 & 2629 & -22 \\
W-score & $J_{.5}$ & 0 & 805 & 412 & 375 & 3093 & 37 \\
W-score & $J_{.5}$ & 1 & 724 & 420 & 399 & 3142 & 21 \\
W-score & $J_{.5}$ & 2 & 758 & 390 & 406 & 3131 & -16 \\
\addlinespace[2pt]
query-only & V & 0 & 1474 & 1374 & 585 & 1252 & 789 \\
query-only & V & 1 & 1469 & 1361 & 590 & 1265 & 771 \\
query-only & V & 2 & 1462 & 1325 & 597 & 1301 & 728 \\
query-only & P & 0 & 2455 & 799 & 403 & 1028 & 396 \\
query-only & P & 1 & 2625 & 624 & 365 & 1071 & 259 \\
query-only & P & 2 & 2675 & 597 & 368 & 1045 & 229 \\
query-only & VP & 0 & 820 & 1193 & 404 & 2268 & 789 \\
query-only & VP & 1 & 886 & 1107 & 421 & 2271 & 686 \\
query-only & VP & 2 & 886 & 1108 & 430 & 2261 & 678 \\
query-only & $VI_{.5}$ & 0 & 4 & 1631 & 3 & 3047 & 1628 \\
query-only & $VI_{.5}$ & 1 & 3 & 1566 & 4 & 3112 & 1562 \\
query-only & $VI_{.5}$ & 2 & 4 & 1562 & 3 & 3116 & 1559 \\
query-only & $J_{.5}$ & 0 & 4 & 1213 & 3 & 3465 & 1210 \\
query-only & $J_{.5}$ & 1 & 3 & 1141 & 4 & 3537 & 1137 \\
query-only & $J_{.5}$ & 2 & 4 & 1144 & 3 & 3534 & 1141 \\
\addlinespace[2pt]
\bottomrule\end{tabular}
\caption{COIN evidence-first, finite reference: all paired four-cell counts for G-score versus each control. Each row sums to 4,685; $\Delta n$ is score-only minus control-only. No case independence or confirmatory significance is inferred.}
\label{tab:coin12-fourcell-Efirst-finite-047}\end{table*}
\FloatBarrier


==> evidence/crosstask_core_results_094.tex <==
\FloatBarrier
\section{CrossTask T3: Complete Three-Seed Native/Query-Only Comparison}
\label{app:ct6-core-094}
\paragraph{Scope and source identity.}
This separate CrossTask~\cite{crosstask2019} instantiation retains 133 raw action
IDs, source spellings and a fixed mixed-candidate, annotation-hull construction.
It is not a reproduction of the old cache's individual case identities or its
FULL-SR results. The benchmark's complete-witness J includes video identity,
IoU-qualified interval and the entire plan under one retained witness.
Six original fits cross G-score/query-only and seeds 0--2 on the same 2,028
exposed VALID cases. The main head is native-joint MAP throughout; evidence-first
is secondary. No per-seed best head, later seed34 expansion or pending selected
planner result enters this comparison. A missing selected-planner result is
not zero and is not represented by a table row.

\paragraph{Source-specific recipe.}
The admission yields 12,858 TRAIN and 2,028 VALID cases from 2,157 and 341
admitted video UIDs, respectively. The public query catalogues contain 858/519
texts (870 in their union). A split hashes video identity modulo 100:
TRAIN uses buckets 15--99 and VALID 0--14. This does not establish an official
or independent test. Literal C133 mappings preserve skipped spelling cases;
they do not silently apply the three proposed alias corrections.
Retained annotations are stable-sorted by start time and original CSV row index;
each consecutive three-row slice defines a complete target tuple.
Candidates contain the source UID, two other same-task UIDs and one other-task
UID, with deterministic case-index-seeded shuffle/positive placement. Candidate
construction is fixed across fitting seeds; task identities use actual task
names/IDs, not the historical all-zero task-class field.

Raw feature files contain preexisting finite FP32 $N\times512$ rows; the
$N\ge16$ admission gate runs before pools, case indices and random calls.
Sixteen rows use rounded linspace indices from 0 to N-1, preserving their original
values. These are not claimed newly extracted InternVideo features. The
reference span uses the minimum start and maximum end of all three annotations,
normalized by the UID's retained annotation extent and mapped to the 16-cell
proxy. It is an annotation-containment construction, not certified media time,
semantic support or uniqueness. Finite witnesses retain all exact same-query
complete video/interval/plan atoms among the four candidates; unannotated
alternatives remain unknown. Both reference policies rescore the same decisions.

\paragraph{Model, control and training.}
The native wrapper fixes $\rho=.5$, $T=3$ and a 133-class
head. Actual source checks show that the global and local routes use the same
projections, encoder and latent cross-attention, both execute, and their pooled
features mix equally before the unchanged output projection/planner.
Query-only zeroes raw visual values in evidence and planning while preserving
the same two-route computation, query, biases, geometry and parameter shapes.
It is a matched visual-input control, not an unadapted historical VSPP system.
Canonical TRAIN full-witness events, not private VALID targets, supply the loss.

Each fit uses fixed 100 epochs, 160,800 optimizer updates and 1,285,800 case exposures,
effective/microbatch 8, hypothesis chunks 16, AdamW learning rate $10^{-4}$,
$(\beta_1,\beta_2)=(.9,.999)$, $\epsilon=10^{-8}$ and weight decay $.01$.
Global gradient clipping is 1; attention uses MATH FP32, AMP/TF32 are disabled,
and numerical thread counts are 1. Epoch-seeded shuffles and seed-matched
initialization contracts are shared within the condition pair. Training
metadata report no VALID model call or VALID-based checkpoint selection.
Interrupted fits resume their original state and optimizer history; fixed-E100
states are not selected by validation. Failed checkpoint/early export/recount
attempts and the G-score seed0 recovery history are retained in the evidence
record; successful recovery does not erase those attempts.

These budgets are source-specific: the old COIN study has 182,000 updates and
different feature/candidate construction. Comparing absolute cross-source
success is not an encoder- or compute-matched transfer study. Main Table~3(b) reports a separate matched CrossTask CM comparison.

\paragraph{CrossTask four-video compatibility.}
We ran the variable-size code at $K=4$ on all 2,028 exposed
validation cases per seed, using the same three final G-score
checkpoints, GPUs and batches as in the original runs.
The six arrays in Table~\ref{tab:ct-k4-saved-fields} and both prediction
heads matched the archive byte for byte in every batch and over the full run.
At $K=6$ and $K=8$, all three checkpoints gave repeatable outputs
on three fixed rows per size. Both heads returned a video, valid interval,
and a complete action sequence. Section~\ref{app:ct-r012-candidate-sensitivity} gives the full candidate-list evaluation.

\begin{table}[!htbp]
\centering\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}ll@{}}
\toprule
Saved field & Value for interval $h$ \\
\midrule
\texttt{E} & Evidence logit $E_h$ \\
\texttt{Z} & Action logits $z_{h,t,a}=Z_\theta(x,h)_{t,a}$ \\
\texttt{LOGPART} & $\sum_{t=1}^T \log\sum_a\exp z_{h,t,a}$ \\
\texttt{RAWBEST} & $\sum_{t=1}^T \max_a z_{h,t,a}$ \\
\texttt{JOINT} & $\log\pi_h+\sum_{t=1}^T\max_a\log p_{h,t}(a)$ \\
\texttt{NATIVE{\char95}ACTIONS} & $\bigl(\arg\max_a z_{h,t,a}\bigr)_{t=1}^T$ \\
\bottomrule
\end{tabular}
\caption{CrossTask T3 saved fields in the four-video check. The code
computes \texttt{JOINT} from log-softmax values. The joint head selects
the interval with the largest \texttt{JOINT}. Evidence-first selects the
interval with the largest \texttt{E}. Both return the selected interval's
saved action sequence.}
\label{tab:ct-k4-saved-fields}
\end{table}

\paragraph{Accepted results and independent recount.}
Tables~\ref{tab:ct6-summary40-094}--\ref{tab:ct6-paired20-094}
report the six original fits. All six original public exports, saved-public QA, private score and distinct
independent exact-Fraction recounts completed. Root acceptance confirms equality
of all 120 integer aggregate totals: six fits, two heads, two reference policies
and five axes. This task did not separately compare every per-case flag, so
aggregate agreement is not described as per-case equality.
The source and immutable old closure roles remain unchanged.

Native-joint finite J is $19.10\pm0.67\%$ for G-score versus
$4.75\pm0.48\%$ for query-only, paired $14.35\pm0.55$ pp.
The three paired changes are 14.45, 14.84, 13.76 pp; no seed is removed.
Finite P changes by only $2.37\pm2.84$ pp on average, including one decrease,
whereas VI/VP/J test support binding. The exact P variation is given by the
paired table below. This supports visual-input value under the declared
protocol; it does not isolate scalar-score fusion, local/global mixing or
causal localization, nor establish superiority to a mature adapted system.
Exposed validation, incomplete witnesses, constructed queries and proxy timing
remain limitations; no held-out or SOTA claim is made.

\begin{table*}[!t]\centering\small\setlength{\tabcolsep}{3pt}\begin{tabular}{lllrrrrr}\toprule Condition & Head & Ref. & V & P & VP & $VI_{.5}$ & $J_{.5}$ \\\midrule
G-score & MAP & can & $37.36\pm1.08$ & $50.23\pm1.72$ & $19.66\pm1.09$ & $19.20\pm0.20$ & $11.14\pm0.30$ \\
G-score & MAP & ann & $54.49\pm0.69$ & $62.87\pm1.28$ & $31.56\pm1.21$ & $31.34\pm0.23$ & $19.10\pm0.67$ \\
G-score & E-first & can & $37.33\pm0.89$ & $49.13\pm2.11$ & $19.26\pm1.32$ & $19.21\pm0.31$ & $10.90\pm0.35$ \\
G-score & E-first & ann & $54.42\pm0.45$ & $61.59\pm1.54$ & $30.79\pm1.68$ & $31.23\pm0.06$ & $18.56\pm0.27$ \\
query-only & MAP & can & $24.79\pm0.10$ & $49.08\pm1.19$ & $11.95\pm0.29$ & $4.77\pm0.47$ & $2.86\pm0.30$ \\
query-only & MAP & ann & $37.25\pm0.22$ & $60.50\pm2.01$ & $19.90\pm0.59$ & $7.41\pm0.72$ & $4.75\pm0.48$ \\
query-only & E-first & can & $24.75\pm0.00$ & $23.90\pm3.21$ & $5.82\pm0.89$ & $0.00\pm0.00$ & $0.00\pm0.00$ \\
query-only & E-first & ann & $37.18\pm0.00$ & $33.79\pm3.30$ & $10.40\pm1.29$ & $0.00\pm0.00$ & $0.00\pm0.00$ \\
\bottomrule\end{tabular}\caption{All 40 CrossTask aggregate metric cells: percent mean $\pm$ sample seed SD, seeds 0--2, $N=2,028$ per seed. Canonical and finite policies evaluate identical predictions.}\label{tab:ct6-summary40-094}\end{table*}
\begin{table*}[!t]\centering\small\setlength{\tabcolsep}{4pt}\begin{tabular}{llrrrrrr}\toprule Condition & Head/ref. & Seed & V & P & VP & $VI_{.5}$ & $J_{.5}$ \\\midrule
G-score & MAP/can & 0 & 765 & 987 & 383 & 385 & 219 \\
G-score & MAP/ann & 0 & 1114 & 1261 & 622 & 632 & 378 \\
G-score & E-first/can & 0 & 752 & 959 & 370 & 386 & 216 \\
G-score & E-first/ann & 0 & 1105 & 1228 & 599 & 634 & 371 \\
G-score & MAP/can & 1 & 733 & 1013 & 389 & 393 & 229 \\
G-score & MAP/ann & 1 & 1089 & 1259 & 630 & 641 & 403 \\
G-score & E-first/can & 1 & 742 & 987 & 381 & 386 & 218 \\
G-score & E-first/ann & 1 & 1094 & 1234 & 611 & 634 & 382 \\
G-score & MAP/can & 2 & 775 & 1056 & 424 & 390 & 230 \\
G-score & MAP/ann & 2 & 1112 & 1305 & 668 & 634 & 381 \\
G-score & E-first/can & 2 & 777 & 1043 & 421 & 397 & 229 \\
G-score & E-first/ann & 2 & 1112 & 1285 & 663 & 632 & 376 \\
query-only & MAP/can & 0 & 505 & 979 & 249 & 88 & 51 \\
query-only & MAP/ann & 0 & 760 & 1200 & 409 & 137 & 85 \\
query-only & E-first/can & 0 & 502 & 534 & 137 & 0 & 0 \\
query-only & E-first/ann & 0 & 754 & 724 & 233 & 0 & 0 \\
query-only & MAP/can & 1 & 501 & 1023 & 240 & 107 & 62 \\
query-only & MAP/ann & 1 & 751 & 1274 & 412 & 166 & 102 \\
query-only & E-first/can & 1 & 502 & 509 & 116 & 0 & 0 \\
query-only & E-first/ann & 1 & 754 & 724 & 218 & 0 & 0 \\
query-only & MAP/can & 2 & 502 & 984 & 238 & 95 & 61 \\
query-only & MAP/ann & 2 & 755 & 1207 & 390 & 148 & 102 \\
query-only & E-first/can & 2 & 502 & 411 & 101 & 0 & 0 \\
query-only & E-first/ann & 2 & 754 & 608 & 182 & 0 & 0 \\
\bottomrule\end{tabular}\caption{All 120 accepted integer counts from six fits, two heads, two policies and five axes, each out of 2,028. This is the full original three-seed cohort.}\label{tab:ct6-count120-094}\end{table*}
\begin{table*}[!t]\centering\small\setlength{\tabcolsep}{4pt}\begin{tabular}{lllrr}\toprule Head & Ref. & Axis & Paired $\Delta$ pp, mean$\pm$SD & Count changes, seeds 0/1/2 \\\midrule
MAP & can & V & $+12.57\pm1.03$ & $+260,+232,+273$ \\
MAP & can & P & $+1.15\pm2.13$ & $+8,-10,+72$ \\
MAP & can & VP & $+7.71\pm1.32$ & $+134,+149,+186$ \\
MAP & can & $VI_{.5}$ & $+14.43\pm0.29$ & $+297,+286,+295$ \\
MAP & can & $J_{.5}$ & $+8.28\pm0.05$ & $+168,+167,+169$ \\
MAP & ann & V & $+17.24\pm0.50$ & $+354,+338,+357$ \\
MAP & ann & P & $+2.37\pm2.84$ & $+61,-15,+98$ \\
MAP & ann & VP & $+11.65\pm1.78$ & $+213,+218,+278$ \\
MAP & ann & $VI_{.5}$ & $+23.93\pm0.49$ & $+495,+475,+486$ \\
MAP & ann & $J_{.5}$ & $+14.35\pm0.55$ & $+293,+301,+279$ \\
E-first & can & V & $+12.57\pm0.89$ & $+250,+240,+275$ \\
E-first & can & P & $+25.23\pm5.30$ & $+425,+478,+632$ \\
E-first & can & VP & $+13.45\pm2.17$ & $+233,+265,+320$ \\
E-first & can & $VI_{.5}$ & $+19.21\pm0.31$ & $+386,+386,+397$ \\
E-first & can & $J_{.5}$ & $+10.90\pm0.35$ & $+216,+218,+229$ \\
E-first & ann & V & $+17.24\pm0.45$ & $+351,+340,+358$ \\
E-first & ann & P & $+27.79\pm4.84$ & $+504,+510,+677$ \\
E-first & ann & VP & $+20.38\pm2.97$ & $+366,+393,+481$ \\
E-first & ann & $VI_{.5}$ & $+31.23\pm0.06$ & $+634,+634,+632$ \\
E-first & ann & $J_{.5}$ & $+18.56\pm0.27$ & $+371,+382,+376$ \\
\bottomrule\end{tabular}\caption{CrossTask T3. All 20 paired G-score-minus-query-only summaries, with all three seed count changes retained. Seed SD describes variation on repeated cases, not a confidence interval; negative and zero changes are not omitted.}\label{tab:ct6-paired20-094}\end{table*}
\FloatBarrier
\subsection{CrossTask candidate-list sensitivity}
\label{app:ct-r012-candidate-sensitivity}
We evaluate three precommitted draws on the same 2,028 exposed validation
cases and the same three frozen G-score checkpoints. Every draw keeps the
same four original videos and their order. We rank the other 337 eligible
video UIDs in the validation pool and append the first two at \(K=6\) or
the first four at \(K=8\). The four-video predictions and success flags
are shared across draws.

The fixed finite policy scores against all complete witnesses in the
original four-video list. The expanded finite policy also includes
complete witnesses from the added videos. Joint success \(J_{.5}\) requires
one witness to support the selected video, interval, and full plan.
Table~\ref{tab:ct-r012-summary} shows how joint success changes as the list
grows. The ranges describe variation across candidate draws on this same
cohort.
Joint success is lower at eight videos than at four for both readouts under both finite reference policies, in every draw and checkpoint.
Section~\ref{app:ct-r012-candidate-audit} gives the draw-level scoring
protocol and the per-checkpoint results, including the canonical policy.

\begin{table}[!ht]
\centering\small
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}lrrrr@{}}
\toprule
Reference & \(K=4\) & \(K=6\) & \(K=8\) & \(\Delta_{4\to8}\) \\
\midrule
\multicolumn{5}{@{}l}{\textbf{Joint MAP}} \\
Fixed & \(19.10\) & \([17.93,18.39]\) & \([16.86,17.41]\) & \([-2.24,-1.69]\) \\
Expanded & \(19.10\) & \([18.24,18.75]\) & \([17.67,17.83]\) & \([-1.43,-1.27]\) \\
\addlinespace[2pt]
\multicolumn{5}{@{}l}{\textbf{Evidence-first}} \\
Fixed & \(18.56\) & \([17.72,17.97]\) & \([16.60,16.95]\) & \([-1.96,-1.61]\) \\
Expanded & \(18.56\) & \([17.90,18.33]\) & \([17.37,17.52]\) & \([-1.18,-1.04]\) \\
\bottomrule
\end{tabular}
\caption{CrossTask T3 joint success \(J_{.5}\) under the fixed and expanded
finite references. Brackets give the observed range of draw means (\%).
\(\Delta_{4\to8}\) is the paired four-to-eight-video change in percentage
points. Each draw mean uses the same three checkpoints.}
\label{tab:ct-r012-summary}
\end{table}
\FloatBarrier

\FloatBarrier
\subsection{CrossTask candidate draw audit}
\label{app:ct-r012-candidate-audit}
For each draw index \(r\in\{0,1,2\}\), we sort the eligible video UIDs by
the SHA-256 digest of the compact UTF-8 JSON array containing, in order,
\texttt{CT\_NESTED\_CANDIDATE\_V1}, the base case ID, the query ID, 4, \(r\),
and the candidate UID. We break ties by UID. The canonical policy uses
one original annotated witness. A separate recount reproduced all
per-case flags in each draw, and the four-video flags match across draws.

Tables~\ref{tab:ct-r012-r0-scores}, \ref{tab:ct-r012-r1-scores}, and
\ref{tab:ct-r012-r2-scores} give success numerators for video (\(V\)), full
plan (\(P\)), video and plan (\(VP\)), video and interval (\(VI_{.5}\)),
and joint success (\(J_{.5}\)). The interval metric uses an IoU threshold
of 0.5. Tables~\ref{tab:ct-r012-r0-paired}, \ref{tab:ct-r012-r1-paired},
and~\ref{tab:ct-r012-r2-paired} give paired joint success flips. Gains
minus losses recover the change in success counts for each seed.
The four-video counts repeat in each score table for direct comparison
within each draw.

\begin{table*}[!htbp]
\centering\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}llrrrrrr@{}}
\toprule
Readout & Reference & \(K\) & \(V\) & \(P\) & \(VP\) & \(VI_{.5}\) & \(J_{.5}\) \\
\midrule
Joint MAP & Canonical & 4 & 765/733/775 & 987/1013/1056 & 383/389/424 & 385/393/390 & 219/229/230 \\
 &  & 6 & 726/693/732 & 1031/1020/1045 & 377/380/398 & 362/360/379 & 207/215/224 \\
 &  & 8 & 689/654/698 & 1027/1015/1038 & 365/353/381 & 351/346/361 & 203/202/214 \\
 & Fixed finite & 4 & 1114/1089/1112 & 1261/1259/1305 & 622/630/668 & 632/641/634 & 378/403/381 \\
 &  & 6 & 1056/1029/1058 & 1282/1270/1296 & 610/597/627 & 591/595/606 & 363/373/364 \\
 &  & 8 & 1003/978/1008 & 1286/1263/1289 & 594/558/598 & 577/569/576 & 363/349/347 \\
 & Expanded finite & 4 & 1114/1089/1112 & 1261/1259/1305 & 622/630/668 & 632/641/634 & 378/403/381 \\
 &  & 6 & 1066/1044/1067 & 1286/1273/1302 & 616/603/633 & 597/606/612 & 366/378/366 \\
 &  & 8 & 1028/1014/1039 & 1300/1273/1301 & 609/572/613 & 593/590/593 & 373/359/353 \\
\midrule
Evidence-first & Canonical & 4 & 752/742/777 & 959/987/1043 & 370/381/421 & 386/386/397 & 216/218/229 \\
 &  & 6 & 717/692/740 & 1003/998/1039 & 366/369/394 & 366/358/378 & 204/206/218 \\
 &  & 8 & 678/651/696 & 995/997/1027 & 347/347/377 & 349/340/360 & 196/194/207 \\
 & Fixed finite & 4 & 1105/1094/1112 & 1228/1234/1285 & 599/611/663 & 634/634/632 & 371/382/376 \\
 &  & 6 & 1053/1025/1063 & 1259/1243/1286 & 594/574/627 & 605/592/603 & 364/356/360 \\
 &  & 8 & 998/970/1004 & 1257/1248/1276 & 571/543/598 & 580/562/568 & 354/338/339 \\
 & Expanded finite & 4 & 1105/1094/1112 & 1228/1234/1285 & 599/611/663 & 634/634/632 & 371/382/376 \\
 &  & 6 & 1061/1039/1071 & 1263/1247/1291 & 599/579/632 & 610/603/609 & 367/360/362 \\
 &  & 8 & 1024/1004/1037 & 1270/1261/1287 & 584/556/614 & 595/583/586 & 363/347/347 \\
\bottomrule
\end{tabular}
\caption{CrossTask draw \(r=0\) success counts. Each cell gives the
counts for seeds 0/1/2, with 2,028 cases per seed. The expanded policy adds
witnesses in 54 cases at \(K=6\) and 115 cases at \(K=8\).}
\label{tab:ct-r012-r0-scores}
\end{table*}

\begin{table*}[!htbp]
\centering\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}llrrrrr@{}}
\toprule
Readout & Reference & Size change & Change (pp) & Gains & Losses & Added-video losses \\
\midrule
Joint MAP & Canonical & \(4\!\to\!6\) & \(-0.53\) & 16/18/20 & 28/32/26 & 12/14/8 \\
 &  & \(6\!\to\!8\) & \(-0.44\) & 13/12/11 & 17/25/21 & 7/15/10 \\
 &  & \(4\!\to\!8\) & \(-0.97\) & 22/17/22 & 38/44/38 & 20/25/17 \\
 & Fixed finite & \(4\!\to\!6\) & \(-1.02\) & 33/29/29 & 48/59/46 & 17/25/15 \\
 &  & \(6\!\to\!8\) & \(-0.67\) & 29/19/20 & 29/43/37 & 14/22/18 \\
 &  & \(4\!\to\!8\) & \(-1.69\) & 45/25/34 & 60/79/68 & 30/44/34 \\
 & Expanded finite & \(4\!\to\!6\) & \(-0.85\) & 35/32/31 & 47/57/46 & 16/23/15 \\
 &  & \(6\!\to\!8\) & \(-0.41\) & 33/22/22 & 26/41/35 & 11/20/16 \\
 &  & \(4\!\to\!8\) & \(-1.27\) & 51/30/38 & 56/74/66 & 26/39/32 \\
\midrule
Evidence-first & Canonical & \(4\!\to\!6\) & \(-0.58\) & 11/12/13 & 23/24/24 & 13/11/7 \\
 &  & \(6\!\to\!8\) & \(-0.51\) & 9/6/5 & 17/18/16 & 6/12/10 \\
 &  & \(4\!\to\!8\) & \(-1.08\) & 16/11/14 & 36/35/36 & 21/21/16 \\
 & Fixed finite & \(4\!\to\!6\) & \(-0.81\) & 29/18/21 & 36/44/37 & 19/23/14 \\
 &  & \(6\!\to\!8\) & \(-0.81\) & 16/9/8 & 26/27/29 & 10/17/19 \\
 &  & \(4\!\to\!8\) & \(-1.61\) & 37/16/21 & 54/60/58 & 31/40/32 \\
 & Expanded finite & \(4\!\to\!6\) & \(-0.66\) & 31/21/23 & 35/43/37 & 18/22/14 \\
 &  & \(6\!\to\!8\) & \(-0.53\) & 20/12/12 & 24/25/27 & 8/15/17 \\
 &  & \(4\!\to\!8\) & \(-1.18\) & 43/21/26 & 51/56/55 & 28/36/29 \\
\bottomrule
\end{tabular}
\caption{CrossTask draw \(r=0\) paired joint success changes. Changes
are means over the three checkpoints in percentage points (pp). Flip counts
are in seed order (0/1/2). A gain changes failure to success and a loss
changes success to failure. Added-video losses also switch the predicted
video to one that was absent from the smaller list.}
\label{tab:ct-r012-r0-paired}
\end{table*}
\FloatBarrier

\begin{table*}[!htbp]
\centering\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}llrrrrrr@{}}
\toprule
Readout & Reference & \(K\) & \(V\) & \(P\) & \(VP\) & \(VI_{.5}\) & \(J_{.5}\) \\
\midrule
Joint MAP & Canonical & 4 & 765/733/775 & 987/1013/1056 & 383/389/424 & 385/393/390 & 219/229/230 \\
 &  & 6 & 713/696/732 & 1014/1038/1035 & 367/384/401 & 362/371/370 & 213/223/224 \\
 &  & 8 & 671/651/681 & 1028/1037/1027 & 358/352/373 & 340/344/349 & 206/203/209 \\
 & Fixed finite & 4 & 1114/1089/1112 & 1261/1259/1305 & 622/630/668 & 632/641/634 & 378/403/381 \\
 &  & 6 & 1040/1032/1046 & 1270/1279/1283 & 592/614/619 & 591/605/595 & 369/386/364 \\
 &  & 8 & 974/983/982 & 1271/1282/1275 & 557/576/579 & 548/573/559 & 343/360/345 \\
 & Expanded finite & 4 & 1114/1089/1112 & 1261/1259/1305 & 622/630/668 & 632/641/634 & 378/403/381 \\
 &  & 6 & 1055/1045/1061 & 1277/1284/1290 & 604/624/628 & 601/614/606 & 378/392/371 \\
 &  & 8 & 1001/1006/1008 & 1284/1292/1284 & 578/591/596 & 567/589/579 & 357/370/357 \\
\midrule
Evidence-first & Canonical & 4 & 752/742/777 & 959/987/1043 & 370/381/421 & 386/386/397 & 216/218/229 \\
 &  & 6 & 700/698/728 & 998/999/1030 & 360/367/400 & 362/364/373 & 211/210/221 \\
 &  & 8 & 654/652/684 & 1009/989/1026 & 342/340/376 & 341/341/352 & 201/194/210 \\
 & Fixed finite & 4 & 1105/1094/1112 & 1228/1234/1285 & 599/611/663 & 634/634/632 & 371/382/376 \\
 &  & 6 & 1029/1036/1044 & 1247/1239/1273 & 577/592/629 & 590/602/597 & 363/367/363 \\
 &  & 8 & 965/981/986 & 1253/1239/1269 & 543/555/585 & 555/570/567 & 342/344/344 \\
 & Expanded finite & 4 & 1105/1094/1112 & 1228/1234/1285 & 599/611/663 & 634/634/632 & 371/382/376 \\
 &  & 6 & 1045/1049/1058 & 1254/1243/1280 & 590/601/638 & 601/611/608 & 373/372/370 \\
 &  & 8 & 993/1003/1012 & 1264/1248/1278 & 563/570/602 & 574/585/587 & 356/354/356 \\
\bottomrule
\end{tabular}
\caption{CrossTask draw \(r=1\) success counts. Each cell gives the
counts for seeds 0/1/2, with 2,028 cases per seed. The expanded policy adds
witnesses in 56 cases at \(K=6\) and 114 cases at \(K=8\).}
\label{tab:ct-r012-r1-scores}
\end{table*}

\begin{table*}[!htbp]
\centering\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}llrrrrr@{}}
\toprule
Readout & Reference & Size change & Change (pp) & Gains & Losses & Added-video losses \\
\midrule
Joint MAP & Canonical & \(4\!\to\!6\) & \(-0.30\) & 19/18/24 & 25/24/30 & 12/13/15 \\
 &  & \(6\!\to\!8\) & \(-0.69\) & 10/6/6 & 17/26/21 & 8/14/8 \\
 &  & \(4\!\to\!8\) & \(-0.99\) & 19/17/21 & 32/43/42 & 19/24/23 \\
 & Fixed finite & \(4\!\to\!6\) & \(-0.71\) & 38/28/34 & 47/45/51 & 19/21/22 \\
 &  & \(6\!\to\!8\) & \(-1.17\) & 14/15/16 & 40/41/35 & 17/20/12 \\
 &  & \(4\!\to\!8\) & \(-1.87\) & 34/31/33 & 69/74/69 & 39/42/33 \\
 & Expanded finite & \(4\!\to\!6\) & \(-0.35\) & 46/30/40 & 46/41/50 & 18/17/21 \\
 &  & \(6\!\to\!8\) & \(-0.94\) & 17/18/20 & 38/40/34 & 15/18/11 \\
 &  & \(4\!\to\!8\) & \(-1.28\) & 45/35/42 & 66/68/66 & 36/36/30 \\
\midrule
Evidence-first & Canonical & \(4\!\to\!6\) & \(-0.35\) & 11/11/21 & 16/19/29 & 8/12/16 \\
 &  & \(6\!\to\!8\) & \(-0.61\) & 6/6/6 & 16/22/17 & 8/12/7 \\
 &  & \(4\!\to\!8\) & \(-0.95\) & 12/12/21 & 27/36/40 & 16/24/23 \\
 & Fixed finite & \(4\!\to\!6\) & \(-0.59\) & 25/20/30 & 33/35/43 & 18/19/25 \\
 &  & \(6\!\to\!8\) & \(-1.04\) & 10/9/9 & 31/32/28 & 18/16/10 \\
 &  & \(4\!\to\!8\) & \(-1.63\) & 25/20/32 & 54/58/64 & 35/37/36 \\
 & Expanded finite & \(4\!\to\!6\) & \(-0.23\) & 33/21/36 & 31/31/42 & 16/15/24 \\
 &  & \(6\!\to\!8\) & \(-0.81\) & 12/12/13 & 29/30/27 & 16/14/9 \\
 &  & \(4\!\to\!8\) & \(-1.04\) & 35/24/41 & 50/52/61 & 31/31/33 \\
\bottomrule
\end{tabular}
\caption{CrossTask draw \(r=1\) paired joint success changes. Changes
are means over the three checkpoints in percentage points (pp). Flip counts
are in seed order (0/1/2). A gain changes failure to success and a loss
changes success to failure. Added-video losses also switch the predicted
video to one that was absent from the smaller list.}
\label{tab:ct-r012-r1-paired}
\end{table*}
\FloatBarrier

\begin{table*}[!htbp]
\centering\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}llrrrrrr@{}}
\toprule
Readout & Reference & \(K\) & \(V\) & \(P\) & \(VP\) & \(VI_{.5}\) & \(J_{.5}\) \\
\midrule
Joint MAP & Canonical & 4 & 765/733/775 & 987/1013/1056 & 383/389/424 & 385/393/390 & 219/229/230 \\
 &  & 6 & 706/693/736 & 995/1026/1044 & 351/371/409 & 368/357/385 & 199/209/226 \\
 &  & 8 & 655/655/679 & 999/1030/1039 & 330/348/379 & 342/336/356 & 188/191/215 \\
 & Fixed finite & 4 & 1114/1089/1112 & 1261/1259/1305 & 622/630/668 & 632/641/634 & 378/403/381 \\
 &  & 6 & 1040/1023/1054 & 1275/1271/1302 & 596/589/636 & 593/583/608 & 356/362/373 \\
 &  & 8 & 970/975/981 & 1269/1284/1294 & 549/562/600 & 560/555/563 & 335/337/354 \\
 & Expanded finite & 4 & 1114/1089/1112 & 1261/1259/1305 & 622/630/668 & 632/641/634 & 378/403/381 \\
 &  & 6 & 1059/1046/1071 & 1284/1286/1315 & 608/604/650 & 604/596/619 & 361/371/381 \\
 &  & 8 & 1008/1017/1022 & 1287/1305/1312 & 573/589/627 & 583/581/587 & 351/355/369 \\
\midrule
Evidence-first & Canonical & 4 & 752/742/777 & 959/987/1043 & 370/381/421 & 386/386/397 & 216/218/229 \\
 &  & 6 & 701/695/727 & 968/1008/1030 & 344/356/401 & 364/362/376 & 199/205/223 \\
 &  & 8 & 654/656/684 & 979/1001/1036 & 324/338/380 & 342/342/350 & 186/185/209 \\
 & Fixed finite & 4 & 1105/1094/1112 & 1228/1234/1285 & 599/611/663 & 634/634/632 & 371/382/376 \\
 &  & 6 & 1041/1027/1047 & 1246/1249/1285 & 582/567/630 & 603/593/599 & 356/352/370 \\
 &  & 8 & 974/973/985 & 1256/1253/1285 & 538/545/603 & 569/562/558 & 336/325/349 \\
 & Expanded finite & 4 & 1105/1094/1112 & 1228/1234/1285 & 599/611/663 & 634/634/632 & 371/382/376 \\
 &  & 6 & 1061/1048/1064 & 1255/1265/1299 & 594/581/645 & 613/605/610 & 361/361/378 \\
 &  & 8 & 1013/1013/1024 & 1275/1276/1304 & 560/572/630 & 592/586/582 & 350/343/364 \\
\bottomrule
\end{tabular}
\caption{CrossTask draw \(r=2\) success counts. Each cell gives the
counts for seeds 0/1/2, with 2,028 cases per seed. The expanded policy adds
witnesses in 73 cases at \(K=6\) and 135 cases at \(K=8\).}
\label{tab:ct-r012-r2-scores}
\end{table*}

\begin{table*}[!htbp]
\centering\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}llrrrrr@{}}
\toprule
Readout & Reference & Size change & Change (pp) & Gains & Losses & Added-video losses \\
\midrule
Joint MAP & Canonical & \(4\!\to\!6\) & \(-0.72\) & 14/14/20 & 34/34/24 & 15/16/11 \\
 &  & \(6\!\to\!8\) & \(-0.66\) & 10/11/15 & 21/29/26 & 9/15/16 \\
 &  & \(4\!\to\!8\) & \(-1.38\) & 17/15/28 & 48/53/43 & 23/30/24 \\
 & Fixed finite & \(4\!\to\!6\) & \(-1.17\) & 34/22/33 & 56/63/41 & 22/31/17 \\
 &  & \(6\!\to\!8\) & \(-1.07\) & 21/18/20 & 42/43/39 & 15/21/24 \\
 &  & \(4\!\to\!8\) & \(-2.24\) & 38/24/43 & 81/90/70 & 40/53/40 \\
 & Expanded finite & \(4\!\to\!6\) & \(-0.81\) & 38/25/38 & 55/57/38 & 21/25/14 \\
 &  & \(6\!\to\!8\) & \(-0.62\) & 30/23/24 & 40/39/36 & 13/17/21 \\
 &  & \(4\!\to\!8\) & \(-1.43\) & 52/32/52 & 79/80/64 & 38/43/34 \\
\midrule
Evidence-first & Canonical & \(4\!\to\!6\) & \(-0.59\) & 11/15/17 & 28/28/23 & 16/17/12 \\
 &  & \(6\!\to\!8\) & \(-0.77\) & 9/10/11 & 22/30/25 & 10/15/16 \\
 &  & \(4\!\to\!8\) & \(-1.36\) & 14/15/22 & 44/48/42 & 25/32/25 \\
 & Fixed finite & \(4\!\to\!6\) & \(-0.84\) & 26/20/29 & 41/50/35 & 22/29/18 \\
 &  & \(6\!\to\!8\) & \(-1.12\) & 17/16/13 & 37/43/34 & 16/22/24 \\
 &  & \(4\!\to\!8\) & \(-1.96\) & 33/21/34 & 68/78/61 & 38/53/41 \\
 & Expanded finite & \(4\!\to\!6\) & \(-0.48\) & 30/23/34 & 40/44/32 & 21/23/15 \\
 &  & \(6\!\to\!8\) & \(-0.71\) & 25/21/17 & 36/39/31 & 14/18/21 \\
 &  & \(4\!\to\!8\) & \(-1.18\) & 45/29/43 & 66/68/55 & 36/43/35 \\
\bottomrule
\end{tabular}
\caption{CrossTask draw \(r=2\) paired joint success changes. Changes
are means over the three checkpoints in percentage points (pp). Flip counts
are in seed order (0/1/2). A gain changes failure to success and a loss
changes success to failure. Added-video losses also switch the predicted
video to one that was absent from the smaller list.}
\label{tab:ct-r012-r2-paired}
\end{table*}
\FloatBarrier


==> evidence/oracle_paired_and_counts.tex <==
\begin{table*}[t]
\centering\small\setlength{\tabcolsep}{5pt}
\begin{tabular}{lllrcrr}
\toprule
$T$/ref. & A & B & B-only & A-only & both/neither & $\Delta J_{.5}$ (pp)\\
\midrule
3/C & Native joint & Oracle video & 177 & 0 & 130/692 & $17.72\pm1.88$ \\
3/C & Native joint & Oracle window & 500 & 0 & 130/369 & $50.05\pm1.42$ \\
3/C & Oracle video & Oracle window & 323 & 0 & 307/369 & $32.33\pm0.87$ \\
4/C & Native joint & Oracle video & 146 & 0 & 85/633 & $16.90\pm0.20$ \\
4/C & Native joint & Oracle window & 335 & 1 & 84/444 & $38.66\pm0.40$ \\
4/C & Oracle video & Oracle window & 189 & 1 & 230/444 & $21.76\pm0.53$ \\
3/$\Omega$ & Native joint & Oracle video & 111 & 64 & 205/619 & $4.70\pm2.72$ \\
3/$\Omega$ & Native joint & Oracle window & 384 & 10 & 259/346 & $37.44\pm1.93$ \\
3/$\Omega$ & Oracle video & Oracle window & 328 & 1 & 315/355 & $32.73\pm0.79$ \\
4/$\Omega$ & Native joint & Oracle video & 99 & 23 & 135/607 & $8.80\pm2.91$ \\
4/$\Omega$ & Native joint & Oracle window & 272 & 7 & 151/434 & $30.67\pm2.63$ \\
4/$\Omega$ & Oracle video & Oracle window & 190 & 1 & 233/440 & $21.88\pm0.35$ \\
\bottomrule\end{tabular}
\caption{Matched G-score paired joint outcomes on all records. B-only are recoveries and A-only regressions when changing A to B. Counts pool 999/864 repeated positions at T3/T4; $\Delta J$ is the mean and sample SD of three paired seed differences, not an unpaired SD or independent-case confidence interval. C/$\Omega$ denote canonical/finite evaluation references. Nonzero regressions remain visible even with privileged geometry.}
\label{tab:p30-oracle-paired}
\end{table*}

\begin{table*}[t]
\centering\small\setlength{\tabcolsep}{3pt}
\begin{tabular}{lllrrrrr}
\toprule
$T$/ref. & Decision & $N$/seed & V & P & VP & $V\mathrm{IoU}_{.5}$ & $J_{.5}$ \\
\midrule
3/C & Native joint & 333 & 99/105/123 & 208/209/215 & 64/64/77 & 61/69/66 & 41/46/43 \\
3/C & Native E-first & 333 & 99/105/123 & 208/209/215 & 64/64/77 & 61/69/66 & 41/46/43 \\
3/C & Oracle video & 333 & 333/333/333 & 207/209/215 & 207/209/215 & 145/149/155 & 95/103/109 \\
3/C & Oracle window & 333 & 333/333/333 & 206/209/215 & 206/209/215 & 333/333/333 & 206/209/215 \\
4/C & Native joint & 288 & 79/95/91 & 135/140/144 & 39/49/52 & 43/52/54 & 22/29/34 \\
4/C & Native E-first & 288 & 79/94/93 & 135/140/144 & 39/49/53 & 43/51/56 & 22/29/35 \\
4/C & Oracle video & 288 & 288/288/288 & 135/139/147 & 135/139/147 & 135/140/140 & 70/78/83 \\
4/C & Oracle window & 288 & 288/288/288 & 134/139/146 & 134/139/146 & 288/288/288 & 134/139/146 \\
\midrule
3/$\Omega$ & Native joint & 333 & 177/182/198 & 231/233/238 & 132/131/141 & 118/119/112 & 90/92/87 \\
3/$\Omega$ & Native E-first & 333 & 177/182/198 & 231/233/238 & 132/131/141 & 118/119/112 & 90/92/87 \\
3/$\Omega$ & Oracle video & 333 & 333/333/333 & 230/233/238 & 211/214/220 & 149/150/160 & 99/104/113 \\
3/$\Omega$ & Oracle window & 333 & 333/333/333 & 229/233/238 & 210/214/220 & 333/333/333 & 210/214/219 \\
4/$\Omega$ & Native joint & 288 & 137/141/147 & 146/149/158 & 84/81/94 & 81/74/88 & 52/43/63 \\
4/$\Omega$ & Native E-first & 288 & 137/140/148 & 146/149/158 & 84/81/94 & 81/73/90 & 52/43/63 \\
4/$\Omega$ & Oracle video & 288 & 288/288/288 & 146/148/161 & 136/140/149 & 138/141/141 & 72/78/84 \\
4/$\Omega$ & Oracle window & 288 & 288/288/288 & 145/148/160 & 135/140/148 & 288/288/288 & 135/140/148 \\
\bottomrule\end{tabular}
\caption{All original records: success numerator triplets in seed order 0/1/2 for all five axes. Each numerator uses the displayed original $N$; failures remain its complement. C/$\Omega$ denote canonical/finite annotation-set references. The counts permit direct reconstruction of means and sample SDs.}
\label{tab:p30-oracle-counts-all}
\end{table*}

\begin{table*}[t]
\centering\small\setlength{\tabcolsep}{3pt}
\begin{tabular}{lllrrrrr}
\toprule
$T$/ref. & Decision & $N$/seed & V & P & VP & $V\mathrm{IoU}_{.5}$ & $J_{.5}$ \\
\midrule
3/C & Native joint & 315 & 94/99/116 & 208/209/213 & 64/64/77 & 60/66/62 & 41/46/43 \\
3/C & Native E-first & 315 & 94/99/116 & 208/209/213 & 64/64/77 & 60/66/62 & 41/46/43 \\
3/C & Oracle video & 315 & 315/315/315 & 207/209/213 & 207/209/213 & 140/145/150 & 95/103/109 \\
3/C & Oracle window & 315 & 315/315/315 & 206/209/213 & 206/209/213 & 315/315/315 & 206/209/213 \\
4/C & Native joint & 265 & 75/88/87 & 135/139/143 & 39/48/52 & 42/49/54 & 22/28/34 \\
4/C & Native E-first & 265 & 75/87/88 & 135/139/143 & 39/48/53 & 42/48/55 & 22/28/35 \\
4/C & Oracle video & 265 & 265/265/265 & 135/138/146 & 135/138/146 & 126/130/134 & 70/77/83 \\
4/C & Oracle window & 265 & 265/265/265 & 134/138/145 & 134/138/145 & 265/265/265 & 134/138/145 \\
\midrule
3/$\Omega$ & Native joint & 315 & 172/176/191 & 231/233/236 & 132/131/141 & 117/116/108 & 90/92/87 \\
3/$\Omega$ & Native E-first & 315 & 172/176/191 & 231/233/236 & 132/131/141 & 117/116/108 & 90/92/87 \\
3/$\Omega$ & Oracle video & 315 & 315/315/315 & 230/233/236 & 211/214/218 & 144/146/155 & 99/104/113 \\
3/$\Omega$ & Oracle window & 315 & 315/315/315 & 229/233/236 & 210/214/218 & 315/315/315 & 210/214/217 \\
4/$\Omega$ & Native joint & 265 & 132/133/142 & 146/148/157 & 84/80/94 & 79/70/88 & 52/42/63 \\
4/$\Omega$ & Native E-first & 265 & 132/132/142 & 146/148/157 & 84/80/94 & 79/69/89 & 52/42/63 \\
4/$\Omega$ & Oracle video & 265 & 265/265/265 & 146/147/160 & 136/139/148 & 129/131/135 & 72/77/84 \\
4/$\Omega$ & Oracle window & 265 & 265/265/265 & 145/147/159 & 135/139/147 & 265/265/265 & 135/139/147 \\
\bottomrule\end{tabular}
\caption{Globally literal-query-seen records: success numerator triplets in seed order 0/1/2 for all five axes. Each numerator uses the displayed original $N$; failures remain its complement. C/$\Omega$ denote canonical/finite annotation-set references. The counts permit direct reconstruction of means and sample SDs.}
\label{tab:p30-oracle-counts-seen}
\end{table*}

\begin{table*}[t]
\centering\small\setlength{\tabcolsep}{3pt}
\begin{tabular}{lllrrrrr}
\toprule
$T$/ref. & Decision & $N$/seed & V & P & VP & $V\mathrm{IoU}_{.5}$ & $J_{.5}$ \\
\midrule
3/C & Native joint & 18 & 5/6/7 & 0/0/2 & 0/0/0 & 1/3/4 & 0/0/0 \\
3/C & Native E-first & 18 & 5/6/7 & 0/0/2 & 0/0/0 & 1/3/4 & 0/0/0 \\
3/C & Oracle video & 18 & 18/18/18 & 0/0/2 & 0/0/2 & 5/4/5 & 0/0/0 \\
3/C & Oracle window & 18 & 18/18/18 & 0/0/2 & 0/0/2 & 18/18/18 & 0/0/2 \\
4/C & Native joint & 23 & 4/7/4 & 0/1/1 & 0/1/0 & 1/3/0 & 0/1/0 \\
4/C & Native E-first & 23 & 4/7/5 & 0/1/1 & 0/1/0 & 1/3/1 & 0/1/0 \\
4/C & Oracle video & 23 & 23/23/23 & 0/1/1 & 0/1/1 & 9/10/6 & 0/1/0 \\
4/C & Oracle window & 23 & 23/23/23 & 0/1/1 & 0/1/1 & 23/23/23 & 0/1/1 \\
\midrule
3/$\Omega$ & Native joint & 18 & 5/6/7 & 0/0/2 & 0/0/0 & 1/3/4 & 0/0/0 \\
3/$\Omega$ & Native E-first & 18 & 5/6/7 & 0/0/2 & 0/0/0 & 1/3/4 & 0/0/0 \\
3/$\Omega$ & Oracle video & 18 & 18/18/18 & 0/0/2 & 0/0/2 & 5/4/5 & 0/0/0 \\
3/$\Omega$ & Oracle window & 18 & 18/18/18 & 0/0/2 & 0/0/2 & 18/18/18 & 0/0/2 \\
4/$\Omega$ & Native joint & 23 & 5/8/5 & 0/1/1 & 0/1/0 & 2/4/0 & 0/1/0 \\
4/$\Omega$ & Native E-first & 23 & 5/8/6 & 0/1/1 & 0/1/0 & 2/4/1 & 0/1/0 \\
4/$\Omega$ & Oracle video & 23 & 23/23/23 & 0/1/1 & 0/1/1 & 9/10/6 & 0/1/0 \\
4/$\Omega$ & Oracle window & 23 & 23/23/23 & 0/1/1 & 0/1/1 & 23/23/23 & 0/1/1 \\
\bottomrule\end{tabular}
\caption{Globally literal-query-unseen records: success numerator triplets in seed order 0/1/2 for all five axes. Each numerator uses the displayed original $N$; failures remain its complement. C/$\Omega$ denote canonical/finite annotation-set references. The counts permit direct reconstruction of means and sample SDs.}
\label{tab:p30-oracle-counts-unseen}
\end{table*}


==> platform_labels280.tex <==
% Generated from the current supplementary dependency graph.
\expandafter\def\csname PlatformSupplementLabel@app:chronov2-global-score\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:coin-guide-r11\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:coin-ps3-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:coin-t3-cm-217\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:coin-train-prior-hold\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:coin-visual-controls\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:coin12-full-047\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:complete-controls178\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:ct6-core-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:endpoint-ce-067\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:experimental-contracts-r16\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:factorized-cm-228\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:final-evidence-298\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:fixed-evidence-composition-076\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:fresh-native-fp32-051\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:full-action-search-r16\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:geometry-threshold-r12\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:h2-latency-051\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:hard-global-cm244-252\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:historical-coverage-086\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:interval-diagnostic-298\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:main-details-002\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:main-display-notes-r15\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:matched-point-095\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:mathematical-analysis-r12\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:mbr-readout-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:media-provenance-067\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:model-details-r11\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:native-matched-cm247-256\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:network-cost302\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:niv-donor-chronological-v2\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:niv-t4-mixing-137\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:p24-global-results\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:p24-retained-window-results\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:p25-followup\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:p26-extra-main-tables\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:p29-external16\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:p30-matched-oracle\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:p33-matched24\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:p34-structured\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:p35-km\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:p3iv-fixed-r-three-arm\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:posterior-allaxes-298\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:posterior-architecture-298\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:posterior-readout-298\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:posterior-risk-298\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:posterior-search-scope-298\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:precision-control-r13\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:proposal-mix-068\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:reference-geometry-324\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:shared-ps-mbr8-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:t4-cm-factorial-201\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:t4-score-access-r16\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:tensor-path-r16\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:train-union178\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@app:uniform-system-067\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:full-action-matrix-r16\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:ma12-compatibility\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:ma12-event-loss\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:ma12-expected-utility\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:ma12-logit-gradient\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:ma12-normalization\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:ma12-normalizers\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:ma12-pool-guarantee\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:ma12-responsibility\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:ma12-total-gradient\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:p23-boundary-token\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:p23-canonical-event\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:p23-global-tokens\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:p25-cell-posterior\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:p25-omega-train\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:posterior-rejection-298\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:posterior-risk-298\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:proposal-local-mix\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:r14-compatible-mass\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@eq:r9-fixed-evidence\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@fig:detailed-routing-r16\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@fig:geometry-threshold-r12\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@fig:implementation-r11\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:SOURCE355_CANONICAL_EFIRST_COMPANION\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:SOURCE355_OMEGA_JOINT_MAIN\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:ab-protocol-adaptation331\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:all144-hard-fiveaxes178\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:all144-semantic-fiveaxes178\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:archive-083\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:candidate-k4\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:chronov2-global-score-paired\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:chronov2-global-score-seed1\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:chronov2-global-score-seed2\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:chronov2-global-score-three-seeds\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:chronov2-literal-strata\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:chronov2-literal-strata-later\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:clip-all5-023\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coin-t3-cm-all-seeds-217\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coin-t3-cm-fiveaxes-217\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coin-t4-first3-retained178\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coin-t4-five-seed178\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coin-train-prior-hold\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coin12-all-summary-047\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coin12-counts-Efirst-047\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coin12-counts-joint-047\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coin12-deltas-Efirst-047\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coin12-deltas-joint-047\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coin12-fourcell-Efirst-canonical-047\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coin12-fourcell-Efirst-finite-047\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coin12-fourcell-joint-canonical-047\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coin12-fourcell-joint-finite-047\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coinps3-count60-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coinps3-pair30-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coinps3-paired10-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coinps3-summary20-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:composition-allhead-summary-076\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:composition-canonical-contrasts-076\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:composition-canonical-seeds-076\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:composition-finite-contrasts-076\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:composition-finite-seeds-076\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:concise-coin-t3\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:concise-coin-t4\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:concise-followup\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:concise-followup-unseen\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:coverage-083\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:ct-t4-first3-retained178\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:ct-t4-five-seed178\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:ct6-count120-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:ct6-paired20-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:ct6-summary40-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:endpoint-ce-counts-067\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:endpoint-ce-summary-067\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:experiment-contracts-current-r16\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:experiment-contracts-retained-r16\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:external-composite303\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:factorized-cm-Jcounts228\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:factorized-cm-allaxes228\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:followup-paired\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:followup-seeds\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:geometry-conquer-t3-r12\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:geometry-conquer-t4-r12\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:geometry-osef-t3-r12\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:geometry-osef-t4-r12\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:h2-latency-051\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:hard-global-cm244-fiveaxes-252\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:hard-global-cm244-pairedJ-252\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:main-supp-map-r16\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:matched-point-seeds-095\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:matched-point-summary-095\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:matched-visual-allstates-007\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:mbr-all60-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:mbr-j-seeds-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:mbr-pairs-0-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:mbr-pairs-1-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:mbr-pairs-2-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:mtid-t4-posthoc\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:native-matched-allaxes247-256\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:native-matched-architecturepairs247-256\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:native-matched-decoderpairs247-256\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:network-cost302\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:niv-donor-v2-all\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:niv-donor-v2-late\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:niv-donor-v2-strata\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:niv-t4-between-137\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:niv-t4-fiveaxes-137\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:niv-t4-union-allfive178\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:niv-t4-within-137\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:notation-main-supp-r16\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p27-fiveaxes\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p29-external-all-canonical\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p29-external-all-omega_ann\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p29-external-literal-query-unseen-canonical\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p29-external-literal-query-unseen-omega_ann\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p30-oracle-counts-all\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p30-oracle-counts-seen\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p30-oracle-counts-unseen\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p30-oracle-paired\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p33-matched24-counts-annotated\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p33-matched24-counts-canonical\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p33-matched24-fiveaxes\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p33-matched24-pairs\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p33-retained-followup\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p33-retained-paired-cost\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p34-structured-J-pairs\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p34-structured-J-seeds\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p34-structured-fiveaxes\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p34-structured-flips\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p34-structured-unseen-counts\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p35-km-fiveaxes\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p35-km-paired\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p3iv-fixed-r-three-arm\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p3iv-seed1-five-axis\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p3iv-seed1-paired\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p3iv-seed2-five-axis\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:p3iv-seed2-paired\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:paired_joint_differences\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:planllm-stage1-v2-posthoc\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:posterior-ct-allaxes-298\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:posterior-native-allaxes-298\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:posterior-paired-J-298\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:posterior-ps-allaxes-298\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:proposal-mix-counts-068\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:proposal-mix-summary-068\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:r13-full-controls-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:retrained-textonly-query10-193\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:sharedps-mbr8-all 40-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:sharedps-mbr8-cross60-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:sharedps-mbr8-crosspairs-0-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:sharedps-mbr8-crosspairs-1-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:sharedps-mbr8-crosspairs-2-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:sharedps-mbr8-crosspairs-3-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:sharedps-mbr8-crosspairs-4-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:sharedps-mbr8-crosspairs-5-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:sharedps-mbr8-pairs-0-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:sharedps-mbr8-pairs-1-094\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:t4-cm-allaxes-201\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:t4-cm-allcontrasts-201\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:t4-score-counts-r16\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:t4-score-pairs-r16\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:t4-score-summary-r16\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:tensor-path-r16\endcsname{1}
\expandafter\def\csname PlatformSupplementLabel@tab:uniform-system-counts-067\endcsname{1}


==> platform_refs280.tex <==
% Loaded after begin-document, after cvpr/cleveref/amsmath label hooks.
\makeatletter
\input{platform_labels280}
\newif\ifPlatformInSupplement
\PlatformInSupplementfalse
\NewCommandCopy{\PlatformOriginalRef}{\ref}
\def\PlatformResolveKey#1{%
  \ifPlatformInSupplement
    \ifcsname PlatformSupplementLabel@#1\endcsname sup-#1\else #1\fi
  \else #1\fi
}
% cleveref routes normal labels and amsmath's packed labels through these two
% literal-key handlers. Namespace before cleveref writes both label and @cref.
\@ifundefined{label@noarg}{\PackageError{arxivassembly}{Required cleveref label hook absent}{}}{}
\let\PlatformOriginalLabelNoarg\label@noarg
\let\PlatformOriginalLabelOptarg\label@optarg
\def\label@noarg#1{%
  \edef\PlatformNext{\noexpand\PlatformOriginalLabelNoarg{\PlatformResolveKey{#1}}}\PlatformNext
}
\def\label@optarg[#1]#2{%
  \edef\PlatformNext{\noexpand\PlatformOriginalLabelOptarg[#1]{\PlatformResolveKey{#2}}}\PlatformNext
}
\RenewDocumentCommand{\ref}{s m}{%
  \edef\PlatformResolvedRef{\PlatformResolveKey{#2}}%
  \IfBooleanTF{#1}{%
    \edef\PlatformNext{\noexpand\PlatformOriginalRef*{\PlatformResolvedRef}}%
  }{%
    \edef\PlatformNext{\noexpand\PlatformOriginalRef{\PlatformResolvedRef}}%
  }\PlatformNext
}
\makeatother


==> platform_setup280.tex <==
% Publication assembly only. Scientific fragments remain byte-identical.
\makeatletter
\newcommand{\PlatformMainPhase}{%
  \global\PlatformInSupplementfalse
  \renewcommand{\theHsection}{main.\arabic{section}}%
  \renewcommand{\theHequation}{main.\arabic{equation}}%
  \renewcommand{\theHfigure}{main.\arabic{figure}}%
  \renewcommand{\theHtable}{main.\arabic{table}}%
  \setcounter{secnumdepth}{2}%
}
\newcommand{\PlatformSupplementLayout}{%
  \renewcommand{\topfraction}{0.95}%
  \renewcommand{\textfraction}{0.05}%
  \renewcommand{\floatpagefraction}{0.7}%
  \renewcommand{\dbltopfraction}{0.95}%
  \renewcommand{\dblfloatpagefraction}{0.7}%
  \setcounter{topnumber}{4}\setcounter{totalnumber}{8}\setcounter{dbltopnumber}{4}%
  \setlength{\@fptop}{0pt}\setlength{\@fpsep}{12pt plus 1fil}%
  \setlength{\@dblfptop}{0pt}\setlength{\@dblfpsep}{12pt plus 1fil}%
  \setcounter{figure}{0}\setcounter{table}{0}\setcounter{equation}{0}\setcounter{footnote}{0}%
  \setcounter{secnumdepth}{3}%
}
\newcommand{\PlatformSupplementPhase}{%
  \global\PlatformInSupplementtrue
  \renewcommand{\theHsection}{supp.\arabic{section}}%
  \renewcommand{\theHequation}{supp.\arabic{equation}}%
  \renewcommand{\theHfigure}{supp.\arabic{figure}}%
  \renewcommand{\theHtable}{supp.\arabic{table}}%
}
\makeatother

